Measuring Neural Net Robustness with Constraints

Despite having high accuracy, neural nets have been shown to be susceptible to adversarial examples, where a small perturbation to an input can cause it to become mislabeled. We propose metrics for measuring the robustness of a neural net and devise a novel algorithm for approximating these metrics based on an encoding of robustness as a linear program. We show how our metrics can be used to evaluate the robustness of deep neural nets with experiments on the MNIST and CIFAR-10 datasets. Our algorithm generates more informative estimates of robustness metrics compared to estimates based on existing algorithms. Furthermore, we show how existing approaches to improving robustness "overfit" to adversarial examples generated using a specific algorithm. Finally, we show that our techniques can be used to additionally improve neural net robustness both according to the metrics that we propose, but also according to previously proposed metrics.

==> discussion.tex <==
\section{Discussion}\label{sec:discuss}

\paragraph{Beyond rectified linear units}
ReLUs allow for a sound and complete characterization of robustness, but other non-linear
layers can be treated just fine, by locally linearizing them, and treating them as linear layers with no constraints.
However, the algorithm has to actually {\em check} if the solver solution is indeed an adversarial example.

\paragraph{Symbolic evaluation and the Jacobian of the model}
Our implementation does not introduce intermediate variables for all layers and input-output equality constraints,
but rather directly propagates linear expressions of the input variables through the layers, implementing a form of
{\em symbolic evaluation} -- this is similar to computing the Jacobian of the model and amenable to GPU-based techniques.

\paragraph{Scalability and performance}
Our {\em refinement} algorithm solves a few 
thousand constraints per iteration -- LP solve time is in the order of 1s for LeNet and 10s 
per image for NiN. To scale to larger inputs (e.g. the ImageNet dataset, 256x256 RGB) we need to apply a similar 
refinement algorithm to gradually introduce {\em variables} in addition to gradually introducing constraints.
Another idea is to apply our methods after the feature extraction layers of a network, where the dimensionality 
is much lower; and use adversaries at that level to fine-tune the classification layers.

\paragraph{Minimizing the loss}
The gradient of the loss is not necessarily aligned
with the direction of the nearest counterexample because this gradient is affected by the confidence.
The more confident a classification is
the more aligned is this gradient with the counterexample direction.
Unfortunately most adversarial examples occur close to the classifier boundary where confidence is
weaker and loss function less smooth. Moreover, it is possible to construct an example where minimizing 
the loss will not succeed in finding an adversarial example.
Consider a classifier $f:\mathbb{R}\to\{0,1,2\}$ defined by the loss function
$J(x,\ell)=
\log\left[\frac{e^{w_{\ell}x+b_{\ell}}}{\sum_{\ell'}e^{w_{\ell'}x+b_{\ell'}}}\right]$
where $\mathbf{w}, \mathbf{b} \in \mathbb{R}^3$, and $w_i$, $b_i$ denote the $i^{th}$ components of 
$\mathbf{w}$ and $\mathbf{b}$ respectively.
Then, $f(x)=\arg\max_{\ell\in\{0,1,2\}}J(x,\ell)$.
%
Consider the case where
$\mathbf{w}^T=\begin{bmatrix}\frac{5}{4} & 1 & 0\end{bmatrix}$, and 
$\mathbf{b}^T=\begin{bmatrix}\log\frac{9}{8} & 0 & \log\frac{1}{3}\end{bmatrix}$.
Let $x_* = 0$ be the seed point. The label at $x_*$ is $\ell_*=f(0)=0$. 
However, the gradient of $J(x,1)$ at $x_* = 0$ is
$(\partial J(x,1)/\partial x)_{x=0}
>0$
Therefore, L-BFGS-B returns $\xopt>0$, but $f(x)=0$ for every $x>0$, so no adversarial example is found.
However, the point $\xadv=-1$ has 
label $\ell=2$, so this is an adversarial example (with $\epsilon=1$).

